HGCLIP: Exploring Vision-Language Models with Graph Representations for Hierarchical Understanding

Object categories are typically organized into a multi-granularity taxonomic hierarchy. When classifying categories at different hierarchy levels, traditional uni-modal approaches focus primarily on image features, revealing limitations in complex scenarios. Recent studies integrating Vision-Language Models (VLMs) with class hierarchies have shown promise, yet they fall short of fully exploiting the hierarchical relationships. These efforts are constrained by their inability to perform effectively across varied granularity of categories. To tackle this issue, we propose a novel framework (HGCLIP) that effectively combines CLIP with a deeper exploitation of the Hierarchical class structure via Graph representation learning. We explore constructing the class hierarchy into a graph, with its nodes representing the textual or image features of each category. After passing through a graph encoder, the textual features incorporate hierarchical structure information, while the image features emphasize class-aware features derived from prototypes through the attention mechanism. Our approach demonstrates significant improvements on 11 diverse visual recognition benchmarks. Our codes are fully available at https://github.com/richard-peng-xia/HGCLIP.

==> main.tex <==
\section{Related Work}
\textbf{Prompt Learning in Vision-Language Models:} 
VLMs leverage information from both image and text modalities to encode multimodal representations. VLMs,  e.g., CLIP~\cite{radford2021learning}, ALIGN~\cite{jia2021scaling}, and LiT~\cite{zhai2022lit} are pre-trained on large-scale image-text pairs and demonstrate remarkable representation abilities on various downstream tasks~\cite{gao2023clip,zhu2022prompt,ding2022decoupling}. However, efficiently adapting them to downstream tasks is still a major challenge. Prompt learning~\cite{li2021prefix,lester2021power}, as a parameter-efficient technique, is well-suited for utilizing the representation capacity of pre-trained VLMs to boost performance, instead of the resource-intensive process of full fine-tuning. Many works~\cite{zhou2022learning,khattak2023maple,xia2023lmpt,shu2022test,zhou2023zegclip,guo2023calip} have demonstrated powerful performance on specific downstream tasks by combining VLMs and prompt tuning. \\
\textbf{Hierarchical Image Classification:} Hierarchical image classification~\cite{salakhutdinov2011learning,guo2018cnn} aims to categorize images into a hierarchical structure that organizes classes into a tree-like taxonomy. It acknowledges the inherent hierarchical nature of visual concepts, allowing for more nuanced and contextually rich image categorization. Prior research has explored various methodologies, including model architectures tailored for hierarchical classification~\cite{guo2018cnn,chang2021your,chen2018fine}, and exploiting the relationship of the categories in the hierarchy~\cite{liu2022focus}. Furthermore, the development of hierarchical classification has spurred some works~\cite{ju2023hierarchical,yi2022exploring} that harness the class hierarchy across diverse domains, as these models tend to focus more on fine-grained and semantically relevant features. Recently, hierarchical labels are integrated with VLMs~\cite{novack2023chils,ge2023improving}. Nonetheless, these methods roughly overlook the hierarchical relationships among labels. Our work \textit{comprehensively} leverages the hierarchical relationships among labels, resulting in performance improvements on \textit{both generic and fine-grained} datasets.\\ 
\textbf{Graph Representation Learning:}\label{sec:grl}
Modern graph analysis methods rely on graph representation learning, encompassing graph embedding, graph neural networks (GNNs), and transformers. Early graph embedding techniques~\cite{perozzi2014deepwalk,grover2016node2vec} typically map nodes into a low-dimensional space, capturing structural information like proximity between nodes~\cite{yu2024few,yu2023generalized}. Recently, GNNs~\cite{kipf2016semi,velivckovic2017graph,yu2023learning} have become the mainstream technique in graph representation learning. They rely on a message-passing framework where each node refines its representation by recursively aggregating messages from its neighbors~\cite{yu2023multigprompt,yu2023hgprompt}. Moreover, some recent approaches have also explored transformer-based architectures~\cite{yun2019graph,hu2020heterogeneous}. Furthermore, the boom of graph representation learning also advances the research and development in other communities such as CV \cite{shi2019skeleton} and NLP \cite{zhang2023pixel}. In this work, we employ \textit{hierarchical graph representations} to enrich multi-modal features, thus improving the model performance and generalization.

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{img/tsne.pdf}
    \caption{t-SNE plots of image embeddings in previous SoTA prompting method CoCoOp, MaPLe, and \model\ on two datasets with distinct semantic granularities. \model\ shows better separability in both fine-grained and coarse-grained levels.}
    \label{fig:tsne}
    % \vspace{-1.5em}
\end{figure*}

\section{Preliminaries}
In this work, our goal is to learn hierarchical multi-modal knowledge via graph encoder based on CLIP. We will introduce related concepts and definitions in the following.
% $\boldsymbol{V}(\cdot)$ $\mathrm{ImageEnc}(\cdot)$ , both of which consist of $Q$ transformer layers $\{\mathcal{I}_{i}\}_{i=1}^Q \{\mathcal{T}_{i}\}_{i=1}^Q$
\subsection{Revisiting CLIP}
\quad We denote the CLIP image and text encoder as $\mathcal{I}(\cdot)$ and $\mathcal{T}(\cdot)$. The dataset contains $K$ categories, \textit{i.e.}, $\{C_1,\cdots,C_K\}$. CLIP leverages a structured approach by inserting all category names into a predefined textual template represented by the \texttt{[CLASS]} token, \textit{e.g.}, creating expressions like “\texttt{a photo of a [CLASS].}". This results in the generation of textual inputs denoted as $T_{K}$. Subsequently, textual features, represented as $\mathbf{F}_{t} \in \mathbb{R}^{K \times D}$, are extracted. Each input image $I$ is divided into $M$ fixed-sized patches, and each patch is embedded into $D$-dimensional latent space. Then CLIP derives its spatial feature map $\mathbf{F}_{s} \in \mathbb{R}^{H \times W \times D}$ and computes the global visual representations $\mathbf{f}_{v} \in \mathbb{R}^{1 \times D}$ through pooling operations, where $H$ and $W$ denote the height and width of the feature map. The integration of features from both encoders is achieved through cosine similarity measures, ultimately yielding classification $logits \in \mathbb{R}^{1 \times K}$. This comprehensive process can be summarized as follows
\begin{equation}
    \mathbf{F}_{t} = \mathcal{T}(T_{K}) ,
\end{equation}
\begin{equation}
    \mathbf{f}_{v} = \textsc{Pooling}(\mathbf{F}_{s}), \quad \textbf{F}_{s} = \mathcal{I}(I),
\end{equation}
\begin{equation}
    \textit{logits} = \mathbf{f}_{v}{\mathbf{F}_{t}}^{T}.
\end{equation}

The matrix multiplication operation between $\mathbf{f}_{v}$ and $\mathbf{F}_{t}$ is equivalent to calculating cosine similarities, assumed to be $L_2$-normalized features. $\textit{logits}$ signifies the computed probabilities for all $K$ categories, and CLIP identifies the category with the maximum output probability $\mathrm{argmax}_{C_K}(\textit{logits})$ as its final prediction.

\subsection{Graph Encoder}
\textbf{Graph.}
A graph is represented as \( G = (V, E) \), with \( V \) denoting the set of nodes and \( E \) the set of edges. 
Equivalently, the graph can be represented by an adjacency matrix $A$, such as $A_{ij}=1$, if $(v_i,v_j) \in E$, for any $v_i,v_j\in V$.\\
\textbf{Graph Encoder.}
GNNs are popular choices of graph encoder, most of which employ a message-passing mechanism \cite{wu2020comprehensive}. Specifically, each node in the graph aggregates messages (\textit{i.e.}, input features or embeddings) from its neighboring nodes to update its own embedding. Multiple layers of neighborhood aggregation can be stacked, facilitating recursive message passing across the graph. 
Formally, in the $l$-th GNN layer, the embedding of node $v$, denoted by $\mathbf{f}^l_v$, is calculated based on the embeddings in the previous layer, as follows
\begin{equation}
    \mathbf{f}^l_v = \textsc{Aggr}(\mathbf{f}^{l-1}_v, \{\mathbf{f}^{l-1}_u : u\in\mathcal{N}_v\}; \theta^l),
\end{equation}
where $\mathcal{N}_v$ is the set of neighboring nodes of $v$, $\theta^l$ is the learnable GNN parameters in layer $l$. $\textsc{Aggr}(\cdot)$ is the neighborhood aggregation function and can take various forms, ranging from the simple mean pooling \cite{kipf2016semi,hamilton2017inductive} to advanced neural networks such as neural attention \cite{velivckovic2017graph} or multi-layer perceptrons \cite{xu2018powerful}. Note that the initial node embedding $\mathbf{f}^0_v$ is simply given by the input feature.
We abstract the multi-layer encoding process as 
\begin{align}
    \mathbf{f}_v = \textsc{GraphEncoder}(\mathbf{f}_v^0,\mathcal{N}_v;\Theta),
\end{align}
where $\Theta=(\theta^1,\ldots,\theta^L)$ is the collection of weights across the layers. Note that graph embedding methods \cite{perozzi2014deepwalk,tang2015line,grover2016node2vec} and graph transformers \cite{yun2019graph,hu2020heterogeneous,ying2021transformers} could also serves as \textsc{GraphEncoder}. 

% \definecolor{customblue}{HTML}{9CC2DD}
% \definecolor{customyellow}{HTML}{FFE699}
\setlength{\fboxsep}{1pt}
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\linewidth]{img/framework.pdf}
    \caption{The pipeline of \model\ for adapting CLIP to hierarchical image classification. We introduce multi-modal hierarchical prompt to learn contextual representations. Then we construct the label hierarchy into a graph, with its nodes representing the textual or image features of each class. Features integrate hierarchical structure information through message passing in the graph encoder. Textual features directly combine hierarchical representations, while image features focus on class-aware prototypes through the attention mechanism.}
    \label{fig:framework}
    % \vspace{-1.5em}
\end{figure*}

\section{Methodology}
\quad In this section, as shown in Figure~\ref{fig:framework}, we present our proposed method, \textit{i.e.}, \model\, for adapting pre-trained VLMs for hierarchical understanding. Our approach aims to enhance the capacity for understanding multiple semantic levels. Most prior approaches focus on single-label classification, whereas hierarchical classification necessitates that the model attends to features relevant to multi-granularity hierarchies. To this end, \model\ entails: \textbf{a)} introducing learnable prompt tokens within multiple transformer blocks in both the visual and textual branches to learn hierarchical contextual representations; \textbf{b)} employing a graph encoder to encode textual features, integrating them with hierarchical structural information; \textbf{c)} utilizing prototype learning to represent image features of each category and similarly modeling them utilizing a graph encoder, thereafter employing the attention mechanism to enable the spatial feature map of images to focus more on class-aware and hierarchy-guided image features.

\subsection{Hierarchy Setting}
\quad The ground truth class hierarchy currently available in a dataset is usually obtained by querying a WordNet~\cite{fellbaum2010wordnet}-like dictionary, but in the real world, our dataset may have no available class hierarchy. In this case, we turn to LLMs, \textit{i.e.}, ChatGPT~\cite{openai2023chat} (GPT-3.5-Turbo), to approximate the hierarchy diagram. Specifically, given some label set size $K$, semantic granularity levels $h$, class names, and optional context, we query ChatGPT with the prompt: \par \texttt{Generate $h$-tier hierarchical labels for the following $K$ \\ categories: $\{C_1,\cdots,C_K\}$.}


\subsection{Multi-modal Hierarchical Prompt}
\quad In order to comprehensively and efficiently leverage the capabilities of pretrained VLMs, we explore the potential of multi-modal prompt, encompassing both textual and visual prompt. As highlighted in~\cite{khattak2023maple}, the acquisition of prompt at deeper transformer layers is crucial, as it progressively models hierarchical feature representations. Learnable tokens are introduced at multiple transformer blocks of both textual and visual branches of VLMs, given as textual prompt $\mathbf{P}^T=\{\mathbf{p}^T_1,\cdots,\mathbf{p}^T_t\}$ and visual prompt $\mathbf{P}^V=\{\mathbf{p}^V_1,\cdots,\mathbf{p}^V_v\}$, respectively. Therefore, the image encoder processes the input tokens added visual prompt $\mathbf{P}^V$ to generate prompted spatial feature map represented as $\tilde{\mathbf{F}_{s}} \in \mathbb{R}^{(HW +v)\times D}$ and prompted global visual representations $\tilde{\mathbf{f}_{v}} \in \mathbb{R}^{1 \times D}$. Similarly, textual prompt $\mathbf{P}^T$ are incorporated into the input tokens for encoding, and textual features are obtained as $\tilde{\mathbf{F}_{t}} \in \mathbb{R}^{K \times D}$. These hierarchical prompt tokens leverage the knowledge encoding capabilities of VLMs to effectively learn task-relevant contextual representations across different semantic levels. 

\subsection{Delving into Graph Representations}
\quad The hierarchical structure among labels naturally forms a tree structure, hence we leverage graph representations to model the hierarchy and integrate it into multi-modal features. In Figure~\ref{fig:tsne}, we visualize and compare the image embeddings of \model\ with those of previous SoTA CoCoOp and MaPLe. It is worth noting that the image embeddings of CLIP, CoOp, CoCoOp, and KgCoOp would be identical, as they do not learn prompts in the visual branch. The visualization reveals that the image embeddings of \model\ are more separable, indicating that incorporating hierarchical information can better adapt CLIP. \\
\textbf{Encoding Text:}
Clearly, textual features $\tilde{\mathbf{F}_{t}}=\{\tilde{\mathbf{f}_{n}^{t}}\}_{n=1}^K$ can be directly employed as input for a graph encoder, as they possess corresponding $D$-dimensional textual features for each category. 
The class hierarchy is constructed into a graph, where vertices and edges represent individual classes and pairs of classes with hierarchical relationships, respectively. As a result, each node $n$ of the text-attributed graph is associated with text features of the corresponding category $\tilde{\mathbf{f}_{n}^{t}}$. The graph encoder approaches node classification by using the structural interactions between nodes. The textual features $\hat{\mathbf{F}_{t}}=\{\hat{\mathbf{f}_{n}^{t}}\}_{n=1}^K$ integrating hierarchical information are encoded as follows:
\begin{equation}
    \{\hat{\mathbf{f}_{n}^{t}}\}_{n=1}^K = \textsc{GraphEncoder}(\tilde{\mathbf{f}_{n}^{t}},\mathcal{N}_n;\Theta_t),
\end{equation}
where $\Theta_t$ denotes the parameters of the graph encoder for textual modality, $\mathcal{N}_n$ denotes the neighbor nodes of $n$. \\
\textbf{Encoding Image:}
In contrast to textual features, the spatial feature map represents the features of each patch, and the global visual representations characterize the image holistically, rather than representing features for each category. Therefore, the image features of each image cannot be directly input into the graph encoder.
\begin{figure}
    \centering
    \vspace{-1em}
    \includegraphics[width=0.5\textwidth]{img/prototypes_.pdf}
    \caption{Semantic prototypes are constructed to guide the learning of hierarchical semantics of images.}
    % \vspace{-1em}
    \label{fig:prototype}
\end{figure}
% \mathbf{F}_{s}^{*}\in \mathbb{R}^{K \times M\times M \times D}
To address this issue, as shown in Figure~\ref{fig:prototype}, we first leverage prototype learning to represent the image features for each category. The global features $\mathbf{F}_{v}^{*}=\{\mathbf{f}_{n}^{v*}\}_{n=1}^K \in \mathbb{R}^{K \times 1 \times D}$ of all images $\{I_{n}\}_{n=1}^K$ (only in the training set) belonging to each class are extracted as prototypes for all categories. These prototypes can then be utilized by the graph encoder to be encoded. The procedure is as follows
\begin{equation}
    \mathbf{F}_{v}^{*} = \textsc{Pooling}(\mathbf{F}_{s}^{*}),\quad \mathbf{F}_{s}^{*} = \mathcal{I}(I_{K}).
\end{equation}

In the image-attributed graph, each node $n$ is associated with image features $\{\mathbf{f}_{n}^{v*}\}_{n=1}^K$, while the rest is consistent with the text-attributed graph. Similarly, the image features $\hat{\mathbf{F}_{v*}}$ are encoded as follows
\begin{align}
    \{\hat{\mathbf{f}_{v*}^{n}}\}_{n=1}^K = \textsc{GraphEncoder}(\mathbf{f}_{v*},\mathcal{N}_n;\Theta_v),
\end{align}
where $\Theta_v$ denotes the parameters of the graph encoder for visual modality. After the visual graph encoder effectively leverages structural knowledge, we then employ the attention mechanism to obtain the attention weights of visual features $\tilde{\mathbf{F}_{s}}$ with respect to the prototypes $\hat{\mathbf{F}_{v*}}$. The calculation of attention weights is as follows
\begin{equation}
    \psi = \tilde{\mathbf{F}_{s}}{{\hat{\mathbf{F}_{v*}}}^T} \in \mathbb{R}^{(HW+v) \times K},
\end{equation}
where $\psi$ denotes the attention map. Each element of $\psi$ represents the attention weight, namely, the feature similarity between a class prototype and one image pixel/site. Based on $\psi$, we update the spatial feature map as follows
\begin{equation}
     \hat{\mathbf{F}_{s}} = \mathrm{SoftMax}(\psi/\alpha)\hat{\mathbf{F}_{v*}},
\end{equation}
where $\alpha$ modulates the attention magnitude. Weighted by the attention scores representing similarity, the image features incorporate structured information from the prototypes. As the prototypes $\hat{\mathbf{F}_{v*}}$ encode $K$-category visual knowledge, the signals of classes appearing in the image would be more notable. Meanwhile, the spatial feature map provides pixel-level fine-grained information for the interaction, contributing to the thorough integration of class-aware features from the prototypes into the image features. \\
\textbf{Classification Logits:} Finally, we obtain the attention-interacted global visual feature by pooling and output the classification logits as
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.5\linewidth]{img/prototypes_.pdf}
%     \caption{Semantic prototypes are constructed to guide the learning of hierarchical semantics of images.}
%     \label{fig:prototype}
%     % \vspace{-1.5em}
% \end{figure}
\begin{equation}
    \hat{\mathbf{f}_{v}} = \textsc{Pooling}(\hat{\mathbf{F}_{s}}) \in \mathbb{R}^{1 \times D},
\end{equation}
\begin{equation}
    \textit{logits} = \lambda_1 \cdot \tilde{\mathbf{f}_{v}}{\hat{\mathbf{F}_{t}}}^{T}+\lambda_2 \cdot \hat{\mathbf{f}_{v}}{\hat{\mathbf{F}_{t}}}^{T},
\end{equation}
where $\lambda_1$ and $\lambda_2$ denote hyper-parameters to control the weight assigned to the $\textit{logits}$ that incorporate structured image features.

For hierarchical image classification, the model is required to simultaneously predict several labels at different granularities. Consequently, it is necessary to partition the predicted $\textit{logits}$ into their respective hierarchical categories $\textit{logits}_i$, with each level corresponding to the ground truth labels $GT_i$, where $i=1,\cdots,h$. The overall loss function can be defined as follows
\begin{equation}
    \mathcal{L} = \sum_{i=1}^{h}w_i\cdot\mathcal{L}_{CE}({GT}_i, \textit{logits}_i),
\end{equation}
where $w_i$ denotes the weights for learning features at different hierarchical levels and $\mathcal{L}_{CE}(\cdot,\cdot)$ represents a cross-entropy loss. A higher $w_i$ prioritizes the learning of features at the $i$-th level, and vice versa.

\section{Experiment}
\subsection{Benchmark Setting}
\textbf{Hierarchical Image Classification:} We consider 11 visual classification datasets, covering a wide range of recognition tasks. These include two general object datasets, CIFAR-100~\cite{krizhevsky2009learning} and Caltech-101~\cite{fei2004learning}; six fine-grained datasets, FGVC-Aircraft~\cite{maji2013fine}, StanfordCars~\cite{krause20133d}, Food-101~\cite{bossard2014food}, Fruits-360~\cite{murecsan2017fruit}, OxfordPets-37~\cite{parkhi2012cats} and ETHEC~\cite{dhall2020hierarchical}; a scene recognition dataset SUN397 \cite{xiao2010sun}; a texture dataset DTD \cite{cimpoi2014describing} and a satellite image dataset EuroSAT \cite{helber2019eurosat}. The aim is to demonstrate our method under general situations of data diversity, where the label hierarchical levels range from two to four. \\
\textbf{Implementation Details:} We use top-1 accuracy to evaluate the prediction performance. We adopt CLIP ViT-B/16 as the visual encoder and use the corresponding CLIP Transformer as the text encoder. We set $\lambda_1$ = 1 and $\lambda_2$ = 0.2 to weight the proportion of hierarchical structural information. For hierarchical classification, we use deep prompting with $v=t=4$ in the first 9 transformer layers and train the models for 50 epochs. All models are trained with a batch size of 64 and a learning rate of 3e-4 via SGD optimizer, and decay by the cosine annealing rule during training. 
\begin{table*}[t]
\centering
\footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{lccccccccc}
\toprule \rowcolor{gray!20}
\multicolumn{2}{l|}{Dataset}  & \begin{tabular}[c]{@{}c@{}}CLIP \\ \textcolor{gray}{\scriptsize \textup{ICML'21}}\end{tabular}  & \begin{tabular}[c]{@{}c@{}}CoOp \\ \textcolor{gray}{\scriptsize \textup{IJCV'22}}\end{tabular} &  \begin{tabular}[c]{@{}c@{}}CoCoOp \\ \textcolor{gray}{\scriptsize \textup{CVPR'22}}\end{tabular} &  \begin{tabular}[c]{@{}c@{}}VPT \\ \textcolor{gray}{\scriptsize \textup{ECCV'22}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}MaPLe \\ \textcolor{gray}{\scriptsize \textup{CVPR'23}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}KgCoOp \\ \textcolor{gray}{\scriptsize \textup{CVPR'23}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}PromptSRC \\ \textcolor{gray}{\scriptsize \textup{ICCV'23}}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\model\\ \textcolor{gray}{\scriptsize \textup{(Ours)}}\end{tabular} \\ \hline \hline 
\multirow{2}{*}{CIFAR-100*}   & \multicolumn{1}{c|}{$l_1$} & 43.22  & 83.76  & 82.60  & 88.75  & \underline{90.67} & 78.65  & 88.18  & \textbf{91.87}  \\
& \multicolumn{1}{c|}{$l_2$} & 66.57  & 76.81  & 75.73  & 83.94  & \underline{85.81} & 73.49  & 82.24  & \textbf{86.55}  \\ \hline
\multirow{3}{*}{Caltech-101} & \multicolumn{1}{c|}{$l_1$} & 58.47  & 96.19  & 96.95 & 96.62  & \underline{98.06}  & 93.50  & 95.70  & \textbf{98.50}   \\
& \multicolumn{1}{c|}{$l_2$} & 69.01  & 95.12  & 94.18 & 95.06  & \underline{97.38}  & 93.56  & 95.57  & \textbf{97.51}   \\
& \multicolumn{1}{c|}{$l_3$} & 84.56  & 95.88  & 95.85 & 96.12  & \underline{96.88}  & 94.81  & 95.51  & \textbf{97.03}   \\ \hline
\multirow{3}{*}{\begin{tabular}[l]{@{}l@{}}FGVC-\\Aircraft*\end{tabular}} & \multicolumn{1}{c|}{$l_1$} & 31.08  & 54.30  & 54.80 & 56.81  & \underline{70.79}  & 53.31  & 55.99  & \textbf{79.24}   \\
& \multicolumn{1}{c|}{$l_2$} & 35.49  & 51.59  & 50.42  & 53.00  & \underline{68.87} & 50.38  & 50.20  & \textbf{70.70}   \\
& \multicolumn{1}{c|}{$l_3$} & 24.69  & 37.74  & 36.10  & 35.00 & \underline{52.58} & 35.56  & 34.21  & \textbf{61.33}   \\ \hline
\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Stanford\\Cars*\end{tabular}} & \multicolumn{1}{c|}{$l_1$} & 61.75  & 82.39  & 83.31  & \underline{83.46}  & 83.35 & 82.78 & 82.85  & \textbf{83.61}  \\
& \multicolumn{1}{c|}{$l_2$} & 63.59  & 73.35  & 73.86  & 76.53  & \underline{76.92} & 69.01 & 73.24  & \textbf{77.84}  \\ \hline
\multirow{2}{*}{Food-101} & \multicolumn{1}{c|}{$l_1$} & 61.38 & 87.04 & 89.13 & \underline{89.28} & 88.16 & 85.18 & 87.37 & \textbf{91.12} \\
& \multicolumn{1}{c|}{$l_2$} & 85.53  & 86.94 & 87.10  & \underline{88.46}  & 88.04 & 86.00 & 86.89 & \textbf{88.73}  \\ \hline
\multirow{3}{*}{Fruits-360} & \multicolumn{1}{c|}{$l_1$} & 75.43  & 93.73  & 99.21 & 99.46  & \underline{99.59} & 90.95  & 94.41  & \textbf{99.71}   \\
& \multicolumn{1}{c|}{$l_2$} & 34.40  & 86.87  & 96.46 & \textbf{98.65}  & 98.31 & 76.43  & 94.60  & \underline{98.51}   \\
& \multicolumn{1}{c|}{$l_3$} & 23.55  & 85.90  & 96.58 & 97.12  & \textbf{97.78} & 72.80  & 92.13  & \underline{97.73}   \\  \hline   
\multirow{2}{*}{\begin{tabular}[l]{@{}l@{}}Oxford\\Pets-37\end{tabular}} & \multicolumn{1}{c|}{$l_1$} & \textbf{99.97}  & 99.86  & 99.86 & \underline{99.92}  & 99.91 & 99.89  & 99.89  & \underline{99.92}   \\
& \multicolumn{1}{c|}{$l_2$} & 88.14  & 91.94  & 91.97 & 91.81 & 92.14 & 91.81  & \underline{92.19}  & \textbf{92.31}   \\ \hline
\multirow{2}{*}{EuroSAT} & \multicolumn{1}{c|}{$l_1$} & 62.97 & 91.50 & 91.77 & 92.41 & \underline{93.03} & 91.38 & 91.96 & \textbf{95.57} \\
& \multicolumn{1}{c|}{$l_2$} & 41.01 & 86.68 & 87.36 & 88.94 & \underline{90.16} & 87.88 & 88.30 & \textbf{92.79}  \\ \hline
\multirow{3}{*}{SUN397*} & \multicolumn{1}{c|}{$l_1$} & 70.29 & 88.01 & 88.60 & \underline{90.82} & 90.59 & 87.62 & 88.18 & \textbf{92.16}   \\
& \multicolumn{1}{c|}{$l_2$} & 63.59 & 84.28 & 84.20 & 86.29 & \underline{86.72} & 85.11 & 85.40 & \textbf{88.39}  \\
& \multicolumn{1}{c|}{$l_3$} & 60.85 & 78.67 & 78.66 & 80.66 & \underline{81.37} & 79.16 & 80.08 & \textbf{83.41} \\  \hline   
\multirow{2}{*}{DTD} & \multicolumn{1}{c|}{$l_1$} & 55.17 & 80.86 & 80.98 & \underline{83.83} & 83.41 & 87.45 & 81.83 & \textbf{86.82}  \\
& \multicolumn{1}{c|}{$l_2$} & 48.09 & 74.60 & 72.19 & 78.34 & \underline{78.36} & 75.68 & 75.79 & \textbf{81.08}  \\ \hline
\multirow{4}{*}{ETHEC*} & \multicolumn{1}{c|}{$l_1$} & 31.12  & 89.45  & 89.61 & 90.87 & \underline{92.17} & 86.03 & 90.64 & \textbf{95.76}   \\
& \multicolumn{1}{c|}{$l_2$} & 2.65  & 85.10  & 86.07 & 86.79  & \underline{89.60} & 83.11  & 87.91  & \textbf{93.40} \\ & \multicolumn{1}{c|}{$l_3$} & 17.94  & 74.67  & 75.02 & 75.81  & \underline{78.48} & 71.33 & 77.46  & \textbf{82.98} \\ & \multicolumn{1}{c|}{$l_4$} & 1.52 & 49.48  & 51.27 & 51.99  & 55.73  & 47.62  & \underline{55.75} & \textbf{60.39}  \\ \bottomrule
\end{tabular}
}
\caption{Top-1 accuracy (\%) comparison on hierarchical image classification of \model\ with previous CLIP-based prompt tuning methods. The best result is \textbf{bold} and the second best is \underline{underlined}. * denotes that the dataset is with available class hierarchy, and hierarchies of others are queried through ChatGPT~\cite{openai2023chat}. $l_i$ represents the classification accuracy at the $i$-th hierarchical level, where a smaller $i$ indicates a coarser granularity level, and vice versa.}
\label{tab:hie}
\end{table*}

\subsection{Hierarchical Image Classification}
\textbf{CLIP-based prompt tuning methods.} Table~\ref{tab:hie} displays the comparative performance of zero-shot CLIP, recent works on prompt learning and \model\ on 11 diverse hierarchical classification datasets. In the case of CLIP, we utilize handcrafted specific prompts designed for each dataset. In comparison with state-of-the-art MaPLe~\cite{khattak2023maple} and PromptSRC~\cite{khattak2023self}, \model\ exhibits improved performance across all levels on all the datasets, with the exception of a slight decline in performance on Fruits-360. With the contribution of graph representations, as opposed to SoTA MaPLe and PromptSRC, \model\ demonstrates superior generalization across multiple hierarchical categories on all the datasets, achieving an absolute average gain of 2.2\% and 5.7\% respectively. \\
\noindent \textbf{CLIP-based feature adaptation methods.} In Table~\ref{tab:feature}, we compare \model\ with prior feature adaption methods based on CLIP. CLIP-Adapter~\cite{gao2023clip} learns two residual-style adapters after CLIP. Tip-Adapter~\cite{zhang2022tip} constructs a key-value cache model by extracting features from few-shot data through CLIP, then views the cache model as a well-performing initialization and fine-tunes the cache keys. CALIP~\cite{guo2023calip} is proposed to boost CLIP performance via a parameter-free attention module between multi-modal representations. In comparison with these feature adaption approaches, \model\ exhibits excellent feature representation capabilities, with an accuracy on CIFAR-100 that is 8.7\%, 6.2\%, and 13.3\% higher than theirs, respectively. \\
\noindent \textbf{Visual-only hierarchical image classification methods.} We have analysed various multi-modal methods above, and to demonstrate the effectiveness of \model, we compare visual-only fine-grained visual classification methods, as shown in Table~\ref{tab:fine}. Our method still achieve a significant advantage. Additionally, the visual-only FGVC methods are more time-consuming compared to ours (100 v.s. 50 training epochs). 

\begin{figure}[htbp]
\makeatletter\def\@captype{table}
    \centering
    \footnotesize
    \begin{tabular}{lcc}
    \toprule
    \multirow{2}{*}{Method}          & \multicolumn{2}{c}{Acc. \%} \\ \cmidrule(r){2-2} \cmidrule(r){3-3}          & $l_1$      & $l_2$      \\
    \midrule
    CLIP~\cite{radford2021learning}~\textcolor{gray}{\scriptsize \textup{ICML'21}} & 43.22      &  66.57    \\
    Linear probe  & 75.60 & 71.27 \\
    CLIP-Adapter~\cite{gao2023clip}~\textcolor{gray}{\scriptsize \textup{IJCV'23}}  & 83.91     & 77.03     \\
    Tip-Adapter~\cite{zhang2022tip}~\textcolor{gray}{\scriptsize \textup{ECCV'22}} & 84.57     & 81.42     \\ 
    CALIP~\cite{guo2023calip}~\textcolor{gray}{\scriptsize \textup{AAAI'23}} & 77.51 & 74.28 \\ \rowcolor{gray!20}
    \model~\textcolor{gray}{\scriptsize \textup{(Ours)}} & \textbf{91.87} & \textbf{86.55} \\ \bottomrule
    \end{tabular}
    \caption{Comparision with CLIP-based feature adaption methods.}
    \label{tab:feature}
\end{figure}
\begin{figure}
    \centering
    \footnotesize
    \begin{tabular}{lcc}
    \toprule
    \multirow{2}{*}{Method}  & \multicolumn{2}{c}{Acc. \%} \\ \cmidrule(r){2-2} \cmidrule(r){3-3} & $l_1$  & $l_2$ \\
    \midrule
    PMG~\cite{du2020fine}~\textcolor{gray}{\tiny \textup{ECCV'20}}  & 87.16 & 83.02 \\
    FGN~\cite{chang2021your}~\textcolor{gray}{\tiny \textup{CVPR'21}}  & 87.88 & 83.60 \\
    GHORD~\cite{zhao2021graph}~\textcolor{gray}{\tiny \textup{CVPR'21}}  & 87.93 & 84.36 \\
    CHRF~\cite{liu2022focus}~\textcolor{gray}{\tiny \textup{ECCV'22}} & 88.67 & 84.91 \\ 
    TFGIC~\cite{xu2023trusted}~\textcolor{gray}{\tiny \textup{AAAI'23}} & 89.20 & 85.17 \\ \rowcolor{gray!20}
    \model~\textcolor{gray}{\tiny \textup{(Ours)}} & \textbf{91.87} & \textbf{86.55}  \\ \bottomrule
    \end{tabular}
    \caption{Comparison with visual-only SoTA FGVC methods.}
    \label{tab:fine}
\end{figure}

\begin{figure}[htbp]
    \centering
    \scriptsize
    \begin{tabular}{ccccccccc}
    \toprule
    \multicolumn{4}{c}{Module} & \multicolumn{2}{c}{CIFAR-100} & \multicolumn{3}{c}{FGVC-Aircraft} \\ \cmidrule(r){5-6}  \cmidrule(r){1-4} \cmidrule(r){7-9}
    \multicolumn{1}{c}{TP}  & \multicolumn{1}{c}{TG}  & \multicolumn{1}{c}{VP}  & \multicolumn{1}{c}{VG} & \multicolumn{1}{c}{$l_1$} & \multicolumn{1}{c}{$l_2$} & \multicolumn{1}{c}{$l_1$} & \multicolumn{1}{c}{$l_2$} & \multicolumn{1}{c}{$l_3$}\\ \midrule
    \ding{55} & \ding{55} & \ding{55} & \ding{55} & 43.22  & 66.57 & 31.08  & 35.49 & 24.69 \\
    \ding{51} & \ding{55} & \ding{55} & \ding{55} & 84.21  & 77.22 & 54.96  & 52.67 & 38.72 \\
    \ding{55} & \ding{55} & \ding{51} & \ding{55} & 84.21  & 77.22 & 56.81  & 53.00 & 35.00 \\
    \ding{51} & \ding{51} & \ding{55} & \ding{55} & 87.42  & 81.24 & 61.56  & 57.90 & 42.83 \\
    \ding{55} & \ding{55} & \ding{51} & \ding{51} & 87.18  & 80.87 & 61.52  & 58.13 & 43.17 \\
    \ding{51} & \ding{55} & \ding{51} & \ding{55} & 90.67  & 85.81 & 70.79  & 68.87 & 52.58 \\
    \ding{51} & \ding{55} & \ding{51} & \ding{51} & 91.28 & 86.04 & 74.61  & 69.27 & 55.66 \\
    \ding{51} & \ding{51} & \ding{51} & \ding{55} & 91.43 & 85.96 & 75.37  & 69.28 & 57.50 \\ \rowcolor{gray!20}
    \ding{51} & \ding{51} & \ding{51} & \ding{51} & \textbf{91.87} &  \textbf{86.55} & \textbf{79.24}  & \textbf{70.70} & \textbf{61.33} \\ \bottomrule 
    \end{tabular}
    \caption{Component Analysis of \model. TP and VP serve as textual and visual prompts. TG and VG denote graph encoder for textual and visual modality.}
    \label{tab:aba}
\end{figure}

\subsection{Ablative Analysis}
\textbf{Components Analysis:} \model\ primarily consists of multi-modal prompts and graph encoders. In Table~\ref{tab:aba}, we ablate on the performance of each module. The prompts facilitate the model in learning hierarchical contextual features, while the graph encoders effectively integrate hierarchical structure information into the feature representations. This enables the model to achieve impressive results across multiple granularities of hierarchical categories. \\
\noindent \textbf{Noisy Hierarchies Queried by Large Language Models:} It is important to note that LLMs may output sub-optimal hierarchical labels. LLMs produce inconsistent hierarchical labels based on a set of input category names or generate hierarchical labels of different levels, leading to certain biases in the model performance. However, even when utilizing the noisy hierarchy, \model\ still enhances accuracy within the original categories in the dataset. 

\section{Conclusion}
In this work, we propose a novel view that combines VLMs with graph representations. Deep prompts are incorporated into the multi-modal branches, allowing VLMs to better learn hierarchical representations. The graph-based hierarchical relationships are encoded into features, strengthening the connection of features across multiple granularities. When integrating image features with graph representation, given that image features are pixel/region-level, prototype learning is employed for class-level image features, which are then fused with the original image features through the attention mechanism. \model\ achieves SoTA results on several hierarchical image classification benchmarks.
\newpage
\section*{Limitations} Although this work has achieved results by utilizing graph representations to characterize hierarchical information, it merely employs a simple graph encoder (such as GCN, GAT, GraphSAGE) to encode structural information. With the advancement of graph learning, it is anticipated that there will be better graph learning methods for representing hierarchical structures, which could further enhance features. We separately employ graph encoders for different modalities, yielding the best performance, outperforming cross-modal graph encoders with shared weights. This may be because current multi-modal models lack the ability to accurately extract features from each modality. With the development of multimodal models, this limitation is expected to be addressed, significantly reducing training time and improving inference speed. Additionally, we leverage multi-modal prompt learning but have not integrated it with graph learning, perhaps combining the two could yield better results.

